Standardization in resource lambda-calculus

The resource calculus is an extension of the lambda-calculus allowing to model resource consumption. It is intrinsically non-deterministic and has two general notions of reduction - one parallel, preserving all the possible results as a formal sum, and one non-deterministic, performing an exclusive choice at every step. We prove that the non-deterministic reduction enjoys a notion of standardization, which is the natural extension with respect to the similar one in classical lambda-calculus. The full parallel reduction only enjoys a weaker notion of standardization instead. The result allows an operational characterization of may-solvability, which has been introduced and already characterized (from the syntactical and logical points of view) by Pagani and Ronchi Della Rocca.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{S.Alves and I. Mackie (Eds.): Second International Workshop\\ on Linearity 2012 (LINEARITY'12).\\
EPTCS 101, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.101.1}{10.4204/EPTCS.101.1}}

